Agriculture-Vision: A Large Aerial Image Database for Agricultural Pattern Analysis

The success of deep learning in visual recognition tasks has driven advancements in multiple fields of research. Particularly, increasing attention has been drawn towards its application in agriculture. Nevertheless, while visual pattern recognition on farmlands carries enormous economic values, little progress has been made to merge computer vision and crop sciences due to the lack of suitable agricultural image datasets. Meanwhile, problems in agriculture also pose new challenges in computer vision. For example, semantic segmentation of aerial farmland images requires inference over extremely large-size images with extreme annotation sparsity. These challenges are not present in most of the common object datasets, and we show that they are more challenging than many other aerial image datasets. To encourage research in computer vision for agriculture, we present Agriculture-Vision: a large-scale aerial farmland image dataset for semantic segmentation of agricultural patterns. We collected 94,986 high-quality aerial images from 3,432 farmlands across the US, where each image consists of RGB and Near-infrared (NIR) channels with resolution as high as 10 cm per pixel. We annotate nine types of field anomaly patterns that are most important to farmers. As a pilot study of aerial agricultural semantic segmentation, we perform comprehensive experiments using popular semantic segmentation models; we also propose an effective model designed for aerial agricultural pattern recognition. Our experiments demonstrate several challenges Agriculture-Vision poses to both the computer vision and agriculture communities. Future versions of this dataset will include even more aerial images, anomaly patterns and image channels. More information at https://www.agriculture-vision.com.

==> IMAGE_TEX/label_freq.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width=\columnwidth]{IMAGES/label_freq.jpg}
\caption{Label size distributions in AgImageNet.}
\label{fig:label_freq}
\end{figure}

==> IMAGE_TEX/mssv.tex <==
\begin{figure}[hbt!]
\centering
\includegraphics[width=\linewidth]{IMAGES/MSSV.png}
\caption{An illustration of our Multi-scale Sliding-window approach in field image evaluation. The original images are branched into three sliding window processing pipelines and later are fed into our model. The output are a collection of all sub-predictions in which they are aggregated into one heat map. Our final predictions are the decisions using a fixed threshold. }
\label{fig:mssv}
\end{figure}

==> IMAGE_TEX/result_vis.tex <==
\begin{figure*}[hbt!]
\centering
\includegraphics[width=\linewidth]{IMAGES/result_vis.jpg}
\caption{This figure shows the DeepLabv3+ weed predictions on some test samples. Left figure is a whole field result. Right figures are the zoom-in views from 4 different results. Ground truth weeds are highlighted in cyan polygons and model predicted weeds are in blue polygons. Field boundaries are shown in yellow polygons. }
\label{fig:result_vis}
\end{figure*}
\vspace{1.2cm}

==> TABLES/complexity_result.tex <==
% \begin{table}[h!]
% \hspace{0.25cm}
% \centering
% \resizebox{0.46\textwidth}{!}{%
%   \begin{tabular}{c|cccc}
%     \hline
%     Backbone    & ResNet-18  & ResNet-34  & ResNet-50  & ResNet-101      \\ \hline
%     mIoU        & 52.01      & 54.76     & 54.05     & \textbf{56.98} \\ \hline
%     \end{tabular}%
% }
% \newline
% \caption{mIoUs of full-field evaluations using DeepLabv3+ with different ResNet backbones.}
% \label{table:complexity_result}
% \end{table}

\begin{table}[h!]
\centering
\resizebox{0.23\textwidth}{!}{%
  \begin{tabular}{r|c}
    \hline
    Backbone    & mIoU (\%) \\ \hline
    ResNet-18  &  \\ 
    ResNet-34  &  \\
    ResNet-50  &  \\
    ResNet-101 & \textbf{} \\ \hline
    \end{tabular}%
}
\caption{mIoUs using our proposed model with different ResNet backbones.}
\label{table:complexity_result}
\end{table}

==> TABLES/field_stats_combine.tex <==
\begin{table}[!t]
\begin{center}
\resizebox{\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|c|c}
\hline
                                  & Train & Val  & Test \\ \hline
\# (Number of) images             & 13817 & 4264 & 5326 \\ \hline 
\# Annotations (weed cluster)           & 13155 & 4109 & 5369 \\
\# Annotations (double plant)           & 7943  & 2826 & 2871 \\
\# Annotations (planter skip)           & 1406  & 436  & 617  \\ \hline \hline
Max. area (weed cluster) ($px^2$) & 512   & 512  & 512  \\
Max. area (double plant) ($px^2$) & 458   & 407  & 468  \\ 
Max. area (planter skip) ($px^2$) & 477   & 411  & 326  \\ \hline
Avg. area (weed cluster) ($px^2$) & 321   & 270  & 340  \\
Avg. area (double plant) ($px^2$) & 108   & 96   & 113  \\ 
Avg. area (planter skip) ($px^2$) & 71    & 94   & 63   \\ \hline
\end{tabular}%
}
\end{center}
\caption{Statistics for the AgriVision dataset. All area values are rounded to the nearest integer.
}
\label{table:field_stats}
\end{table}


==> TABLES/rgbn_result.tex <==
% \begin{table}[h!]
% \hspace{1cm}
% \centering
% \resizebox{0.23\textwidth}{!}{%
%   \begin{tabular}{c|cc}
%     \hline
%     Channels    & RGB     & NRGB              \\ \hline
%     mIoU        & 55.21  & \textbf{56.98}   \\ \hline
%     \end{tabular}%
% }
% \newline
% \caption{mIoUs of full-field evaluations using DeepLabv3+ trained on RGB images and on NIR-Red-Green-Blue (NRGB) images.}
% \label{table:rgbn_result}
% \end{table}

\begin{table}[h!]
\centering
\resizebox{0.2\textwidth}{!}{%
  \begin{tabular}{r|c}
    \hline
    Channels & mIoU (\%) \\ \hline
    RGB      & \\
    NRG      & \\
    NRGB     & \textbf{} \\ \hline
    \end{tabular}%
}
\caption{mIoUs of field evaluations of our model trained on RGB images and on NIR-Red-Green-Blue (NRGB) images.}
\label{table:rgbn_result}
\end{table}

% \begin{table}[h!]
% \centering
% \resizebox{0.30\textwidth}{!}{%
%   \begin{tabular}{cccc|c}
%     \hline
%     NIR   & Red   & Green & Blue  & mIoU  \\ \hline
%     \tick &       &       &       &       \\ 
%           & \tick &       &       & 49.77 \\ 
%           &       & \tick &       & 49.77 \\ 
%           &       &       & \tick &       \\
%           & \tick & \tick & \tick & 55.21 \\
%     \tick & \tick & \tick & \tick & 56.98 \\
%     \hline
%     \end{tabular}%
% }
% \newline
% \caption{The mIoUs of full-field evaluations using DeepLabv3p-mc trained on RGB images and on NIR-Red-Green-Blue (NRGB) images.} 
% \label{table:rgbn_result}
% \end{table}

==> TABLES/subsampling_result.tex <==
\begin{table}[h!]
\hspace{0.25cm}
\centering
\resizebox{0.43\textwidth}{!}{%
  \begin{tabular}{cccc|c}
    \hline
    Crop1024 & Crop-ms & OS=16 & OS=8  & mIoU           \\ \hline
    \checkmark    &         & \checkmark &       & \textbf{56.98} \\ 
    \checkmark    &         &       & \checkmark & 54.12          \\ 
             & \checkmark   & \checkmark &       & 55.99          \\ 
             & \checkmark   &       & \checkmark & 55.65          \\ \hline
    \end{tabular}%
}
\newline
\caption{mIoUs of multi-channel DeepLabv3+ trained using the two sub-sampling methods with different output strides (OS). } 
\label{table:subsampling_result}
\end{table}

==> TABLES/transfer_result.tex <==
% \begin{table}[h!]
% \hspace{0.5cm}
% \centering
% \resizebox{0.46\textwidth}{!}{%
%   \begin{tabular}{c|ccc}
%     \hline
%     Init method & From Scratch & ImageNet (Xrgb) & ImageNet (rrgb)   \\ \hline
%     mIoU        &        51.50 &           54.73 & \textbf{56.98}   \\ \hline
%     \end{tabular}%
% }
% \newline
% \caption{The mIoUs of full-field evaluations using DeepLabv3+ trained from scratch vs. fine-tuned on the ImageNet pre-trained weights. ImageNet (Xrgb) means the model weights corresponding to the NIR channel are random normal-initialized while ImageNet (rrgb) means those weights are duplicated from the Red.}
% \label{table:transfer_result}
% \end{table}


\begin{table}[h!]
\hspace{0.75cm}
\centering
\resizebox{0.25\textwidth}{!}{%
  \begin{tabular}{r|c}
    \hline
    Init method     &  mIoU \\ \hline
    From Scratch    & 51.50 \\ 
    ImageNet (Xrgb) & 54.73 \\ 
    ImageNet (rrgb) &  \textbf{56.98} \\ \hline
    \end{tabular}%
}
\newline
\caption{mIoUs of field evaluations using DeepLabv3+ trained from scratch vs. fine-tuned on the ImageNet pre-trained weights. ImageNet (Xrgb) means the model weights corresponding to the NIR channel are random normal-initialized. ImageNet (rrgb) means NIR weights are duplicated from the Red channel.}
\label{table:transfer_result}
\end{table}
